AdaTranS: Adapting with Boundary-based Shrinking for End-to-End Speech Translation

To alleviate the data scarcity problem in End-to-end speech translation (ST), pre-training on data for speech recognition and machine translation is considered as an important technique. However, the modality gap between speech and text prevents the ST model from efficiently inheriting knowledge from the pre-trained models. In this work, we propose AdaTranS for end-to-end ST. It adapts the speech features with a new shrinking mechanism to mitigate the length mismatch between speech and text features by predicting word boundaries. Experiments on the MUST-C dataset demonstrate that AdaTranS achieves better performance than the other shrinking-based methods, with higher inference speed and lower memory usage. Further experiments also show that AdaTranS can be equipped with additional alignment losses to further improve performance.

==> figs/diff_nmt.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{figs/diff_nmt1.pdf}
% \vskip -1em
\caption{
Model performance differences between using multi-task learning (MTL) with MT or not when using different amount of extra MT data for pre-training. We share the parameters of the ST semantic encoder and decoder with the MT encoder and decoder.
}
% \vskip -1em
\label{fig:diff_nmt}
\end{figure}

==> figs/intro.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{figs/intro1.pdf}
\vskip -0.5em
\caption{
Modality gap exists when inheriting knowledge from the pre-trained ASR and MT models.
}
\vskip -1em
\label{fig:intro}
\end{figure}

==> sections/related-work.tex <==
\input{figs/architecture}
\section{Related Work}
The earliest ST systems depend on cascading an ASR system and an MT system to perform the translation~\cite{DBLP:conf/icassp/Ney99,DBLP:conf/icassp/MathiasB06,sperber-etal-2017-neural}. Such cascaded systems can leverage the off-the-shelf models and therefore make use of much extra ASR and MT data. Nonetheless, they suffer from the problems of error propagation and high latency~\cite{DBLP:journals/corr/WeissCJWC17}.

End-to-end ST models are proposed to address these drawbacks and have been shown promising recently~\cite{DBLP:journals/corr/BerardPSB16,DBLP:conf/icassp/BerardBKP18,DBLP:conf/interspeech/BansalKLLG18}. However, the data scarcity problem prevents the end-to-end models from being well-trained. Various techniques are explored to alleviate that, like pre-training~\cite{bansal-etal-2019-pre,xu-etal-2021-stacked}, multi-task learning~\cite{DBLP:journals/corr/WeissCJWC17,tang-etal-2021-improving}, knowledge distillation~\cite{DBLP:conf/interspeech/LiuXZHWWZ19,ren-etal-2020-simulspeech}, and data augmentation~\cite{DBLP:conf/icassp/JiaJMWCCALW19,DBLP:conf/interspeech/PinoXMDT20}.

Recently, researchers explore how to adapt the speech and text representations to bridge the modality gap so that ST models can better inherit knowledge from pre-trained models. \citet{DBLP:conf/aaai/WangWLY020} add noises to the text input and \citet{tang-etal-2021-improving,DBLP:conf/icassp/TangPWMG21} represent text input as phoneme sequences to reduce the differences between speech and text input. \citet{wang-etal-2020-curriculum} use a curriculum pre-training procedure to learn cross-lingual information. \citet{han-etal-2021-learning} introduce a shared semantic space for both speech and text, while \citet{xu-etal-2021-stacked} explore using CTC posterior embeddings as input for the semantic encoder. 
Besides, different shrinking mechanisms are proposed to close the length gap~\cite{DBLP:journals/corr/abs-2009-09737,dong2021unist,DBLP:journals/corr/abs-2010-14920,gaido-etal-2021-ctc,zeng-etal-2021-realtrans}. However, they might introduce extra cost and only achieve sub-optimal shrinking results. In this work, we propose an improved shrinking mechanism that can help better inherit knowledge from pre-trained models.

==> tables/ablation.tex <==
\begin{table}[t]
\small
\begin{center}
\setlength{\tabcolsep}{4.0mm}
\begin{tabular}{l|c c }
\toprule[1pt]
\multirow{2}{*}{\bf{Method}} & \multicolumn{2}{c}{\bf BLEU} \\
& En-De & En-Fr \\
\midrule[0.5pt]
Full Model & 28.1 & 38.4 \\
$\;\;$ - CTR & 27.8 & 38.1 \\
$\;\;$ - KD & 26.0 & 37.2 \\
$\;\;$ - CTR - KD & 26.7 & 37.4 \\
\midrule[0.5pt]
$\;\;\;\;$ - Forced Training & 26.4 & 37.1 \\
$\;\;\;\;\;\;$ - Blank Label & 26.3 & 36.6 \\
$\;\;\;\;\;\;\;\;$ - NMT PT & 25.5 & 36.2 \\
$\;\;\;\;\;\;\;\;\;\;$ - ASR PT & 24.5 & 35.0 \\

\bottomrule[1pt]
\end{tabular} 
\end{center}
\vskip -1.0em
\caption{
Ablation study on MUST-C En-De and En-Fr.}
\vskip -1.0em
\label{tab:ablation}
\end{table}

==> tables/acoustic_enc.tex <==
\begin{table}[t]
\small
\begin{center}
\setlength{\tabcolsep}{1.2mm}
\begin{tabular}{l | c | c | c c c}
\toprule[1pt]
\bf{Acoustic} & \multirow{2}{*}{\bf{\#Params}} & \bf{ASR}& \multicolumn{3}{c}{\bf ST BLEU}\\
\bf{Encoder} & & \bf{WER} & ST-B & CTC-Shr & AdaTranS \\
\midrule[0.5pt]
ConvT & 106.2M & 11.2 & 26.0 & 26.4 & 26.7 \\
$\;\;$- Rel & 103.1M & 12.0 & 25.6 & 26.2 & 26.6 \\
S2T & 93.5M & 11.7 & 25.1 & 25.5 & 25.8 \\
CFM & 131.6M & 12.0 & 26.8 & 26.8 & 27.4\\
\bottomrule[1pt]
\end{tabular} 
\end{center}
\vskip -1.0em
\caption{
Results of using different acoustic encoders. ST-B indicates the ST baseline without any shrinking, while CTC-Shr is the CTC-based shrinking method. 
% ``- Rel'' denotes to remove the relative positional encoding.
}
\vskip -1.5em
\label{tab:acoustic-enc}
\end{table}

==> tables/alignment.tex <==
\begin{table}[ht]
\small
\begin{center}
\setlength{\tabcolsep}{1.3mm}
\begin{tabular}{l|c c| c c }
\toprule[1pt]
\multirow{2}{*}{\bf{Method}} & \multicolumn{2}{c|}{\bf With MTL} &\multicolumn{2}{c}{\bf W/O MTL} \\
& En-De & En-Fr & En-De & En-Fr \\
\midrule[0.5pt]
Our Model (AdaTranS) & 25.2 & 30.5 & 25.3 & 30.5 \\
$\;\;$ + KD & 25.8 & 30.9 & 26.8 & 31.4 \\
$\;\;\;\;$ + CAR & 25.9 & 31.1 & 26.9 & 31.6 \\
$\;\;\;\;$ + CMA & 26.1 & 31.0 & 27.0 & 31.4 \\
$\;\;\;\;$ + CTR (Ours) & 25.9 & 31.1 & 27.4 & 31.8 \\
\bottomrule[1pt]
\end{tabular} 
\end{center}
\vskip -1.0em
\caption{
BLEU scores of different encoder output alignment objectives on MUST-C En-De and En-Fr dev set.}
\vskip -1.0em
\label{tab:alignment}
\end{table}

==> tables/main_comparison.tex <==
\begin{table*}[t]
\small
\begin{center}
\setlength{\tabcolsep}{1.7mm}
\begin{tabular}{l|c c c|c|l l l c}
\toprule[1pt]
\multirow{2}{*}{\bf{Model} (Re-implementation)} & \multicolumn{3}{c|}{\bf{Modality Adaptation}} & \multirow{2}{*}{\bf{\#Params}} &  \multicolumn{4}{c}{\bf BLEU} \\
& \bf{Shrink} & \bf{Enc. Align} & \bf{Dec. Align} & & En-De & En-Fr & En-Ru & Avg. \\
% & En-De & En-Es & En-Fr & Model Size & Inference Speedup\\
\midrule[0.5pt]
MT & -- & -- & -- & -- & 34.4 & 44.9 & 21.3 & 33.5 \\
\midrule[0.5pt]
Cascaded Model & -- & -- & -- & 147.5M & 28.1 & 37.0 & 17.6 & 27.6  \\
E2E ST Baseline & -- & -- & -- & 106.2M & 26.0 &  36.8 & 17.0 & 26.6  \\
\midrule[0.5pt]
JT-S-MT~\cite{tang-etal-2021-improving} & $\times$ & CAR & KD & 106.2M & 27.0$^{\dagger}$ & 37.8$^{\dagger}$ & \underline{18.2}$^{\dagger}$ & 27.7   \\
Chimera~\cite{han-etal-2021-learning} & $\times$ & BMC & KD & 115.7M & 27.5$^{\dagger}$ & 38.0$^{\ddagger}$ & 18.0$^{\dagger}$ & 27.8 \\
SATE~\cite{xu-etal-2021-stacked} & $\times$ & CSE & KD  & 114.6M & \underline{27.7}$^{\ddagger}$ & 37.2$^{\dagger}$ & 18.1$^{\dagger}$ & 27.6 \\
UniST~\cite{dong2021unist} & CIF-Based & $\times$ & KD &  106.2M & \underline{27.7}$^{\ddagger}$ & 37.4$^{\dagger}$ & 17.8$^{\dagger}$ & 27.6 \\
STAST~\cite{DBLP:journals/corr/abs-2010-14920} & CTC-Based & CMA & KD  & 114.6M & 27.6$^{\dagger}$ & \underline{38.1}$^{\ddagger}$ & \underline{18.2}$^{\dagger}$ & \underline{28.0}  \\
AdaTranS & Boundary-Based & CTR & KD & 107.0M & \textbf{28.1} & \textbf{38.4} & \textbf{18.7}  & \textbf{28.4}\\
\bottomrule[1pt]
\end{tabular} 
\end{center}
\vskip -1.0em
\caption{
Comparisons on the MUST-C datasets. We re-implement the methods and compare them in a fair situation, including using the same extra data and pre-trained modules. ``CAR'', ``CMA'', ``BMC'' and ``CSE'' are proposed by the corresponding works, short for ``cross-attentive regularization'', ``cross-modal adaptation'', ``bi-modal contrastive'' and ``CTC-based soft embeddings'', respectively. Our AdaTranS significantly outperforms other adaptation methods under paired bootstrap resampling significance test with $p \leq 0.05$ (marked with $^{\ddagger}$) or $p \leq 0.01$ (marked with $^{\dagger}$).}
\vskip -1.0em
\label{tab:main-compare}
\end{table*}


% \begin{table*}[t]
% \small
% \begin{center}
% \setlength{\tabcolsep}{3.3mm}
% \begin{tabular}{l|c c|c|c|c }
% \toprule[1pt]
% \multirow{2}{*}{\bf{Method}} & \multicolumn{2}{c|}{\bf BLEU} & \multirow{2}{*}{\bf{\#Params}} & \multirow{2}{*}{\bf{Speedup}} & \multirow{2}{*}{\bf{Mem Usage}}\\
% & En-De & En-Fr & & &\\
% % & En-De & En-Es & En-Fr & Model Size & Inference Speedup\\
% \midrule[0.5pt]
% MT & 34.4 & 44.9 & -- & -- & --\\
% Cascaded Model & 28.1 &  37.0 & 147.5M & 0.60$\times$ & -- \\
% E2E ST Baseline & 26.0 &  36.8 & 106.2M & 1.00$\times$ & 1.00 \\
% \midrule[0.5pt]
% NMT MTL + CAR + KD~\cite{tang-etal-2021-improving} & 27.0 & 37.8 & 106.2M & 1.00$\times$ & 1.00 \\
% Shared Semantic Space + KD~\cite{han-etal-2021-learning} & 27.5 & 38.0 & 115.7M & 1.04$\times$ & 0.80 \\
% CTC Posterior Embed + KD~\cite{xu-etal-2021-stacked} & 27.7 & 37.2 & 114.6M & 0.73$\times$ & 1.72\\
% \midrule[0.5pt]
% CTC-Based Shrink~\cite{DBLP:journals/corr/abs-2010-14920} & 26.4 & 36.9 & 114.6M & 0.76$\times$ & 1.77 \\
% Weighted Shrink~\cite{zeng-etal-2021-realtrans} & 26.3 & 36.8 & 114.6M & 0.76$\times$ & 1.67 \\
% CIF-Based Shrink~\cite{dong2021unist} & 26.3 & 36.8 & 106.2M & 1.04$\times$ & 0.74 \\
% Boundary-Based Shrink (AdaTranS) & \textbf{26.7} & \textbf{37.4}  & 107.0M & 1.06$\times$ & 0.78 \\
% $\;\;$+ CTR + KD & \textbf{28.1} & \textbf{38.4} & 107.0M & 1.06$\times$ & 0.78 \\
% \bottomrule[1pt]
% \end{tabular} 
% \end{center}
% \vskip -1.0em
% \caption{
% Comparisons on the test set of the two language pairs among different adapt methods. We re-implement all the methods and compare them in a fair situation, including using the same data and model architecture. The speedup and memory usage are both test during inference with a batch size of 16, and we only display the relative values for clear comparison.}
% \vskip -1.0em
% \label{tab:main-compare}
% \end{table*}
